Self-Explaining Neural Networks for Business Process Monitoring

Tasks in Predictive Business Process Monitoring (PBPM), such as Next Activity Prediction, focus on generating useful business predictions from historical case logs. Recently, Deep Learning methods, particularly sequence-to-sequence models like Long Short-Term Memory (LSTM), have become a dominant approach for tackling these tasks. However, to enhance model transparency, build trust in the predictions, and gain a deeper understanding of business processes, it is crucial to explain the decisions made by these models. Existing explainability methods for PBPM decisions are typically *post-hoc*, meaning they provide explanations only after the model has been trained. Unfortunately, these post-hoc approaches have shown to face various challenges, including lack of faithfulness, high computational costs and a significant sensitivity to out-of-distribution samples. In this work, we introduce, to the best of our knowledge, the first *self-explaining neural network* architecture for predictive process monitoring. Our framework trains an LSTM model that not only provides predictions but also outputs a concise explanation for each prediction, while adapting the optimization objective to improve the reliability of the explanation. We first demonstrate that incorporating explainability into the training process does not hurt model performance, and in some cases, actually improves it. Additionally, we show that our method outperforms post-hoc approaches in terms of both the faithfulness of the generated explanations and substantial improvements in efficiency.

==> SECTIONS/related_art.tex <==
\section{Related Work}

\label{sec:related_art}

\subsection{eXplainable Artificial Intelligence}


Given the ``black-box'' nature of modern AI models, the field of \acrshort{xai} \cite{meske2022explainable,adadi2018peeking,arya2019one} aims to address these challenges by providing explanations for \acrshort{ai} model predictions in a way that humans can understand. 
This is particularly crucial in high-stakes applications where decisions may have significant individual or societal consequences, such as those in the judicial, healthcare, or financial domains \cite{jia2022role,marques2022delivering}.


%Due to the ``black-box'' nature of contemporatry AI models, the field of \acrshort{xai}~\cite{meske2022explainable,adadi2018peeking, arya2019one} focuses on mitigating some of these challenges obtaining explanations for the predictions of \acrshort{ai} models to humans. This is especially imperative in high-stakes applications with potentially severe individual or societal consequences (e.g., judicial, health-related, or financial decisions)~\cite{jia2022role,marques2022delivering}.

Traditional post-hoc explainability techniques, such as LIME~\cite{ribeiro2016should} and SHAP~\cite{lundberg2017unified}, generate \emph{additive} feature attributions by assigning importance weights to individual features. These approaches inherently assumes that the model behaves approximately linearly in the vicinity of the input of interest~\cite{yeh2019fidelity}. To bridge this gap, approaches like Anchors~\cite{ribeiro2018anchors} and SIS~\cite{carter2019made} offer an alternative form of explanation by identifying minimal subsets of input features that are independently sufficient to determine the model’s prediction.

%Classic post-hoc explainability approaches such as LIME~\cite{ribeiro2016should} and SHAP~\cite{lundberg2017unified} obtain \emph{additive} feature attributions, by assigning importance weights to individual features and hence rely on an implicit assumption of the model havin near-linear in a local area aroung the input of interest~\cite{yeh2019fidelity}. Following these works, methods such as Anchors~\cite{ribeiro2018anchors}, and SIS~\cite{carter2019made} aim to provide a distinct form of explanation by obtaining minimal subsets of input features that by themselves are sufficient to determine the prediction. 


The literature has proposed various types of sufficient explanations, including those that provide different robustness guarantees~\cite{wu2024verix,marques2022delivering,bassan2023towards,la2021guaranteed,darwiche2020reasons}, probabilistic assurances~\cite{waldchen2021computational,arenas2022computing}, or those that use a specific baseline for evaluating the sufficiency of the subset in question~\cite{chockler2021explanations}. 
While many of these methodologies are model-agnostic, meaning they can be applied across different models, some are designed specifically for particular models like \acrshortpl{DT}~\cite{izza2020explaining}, \acrshort{tf} ensembles~\cite{ignatiev2022using}, or Neural Networks~\cite{wu2024verix,bassan2023towards,la2021guaranteed}.

%Many other forms of sufficient explanations were suggested in the literature, including forms that satisfy different robustness guarantees~\cite{wu2024verix,marques2022delivering,bassan2023towards,la2021guaranteed,darwiche2020reasons}, probabilistic guarantees~\cite{waldchen2021computational,arenas2022computing}, or by using some given baseline to measure the sufficiency of the underlying subset~\cite{chockler2021explanations}. While many of these methods are model-agnostic (i.e., can work for any model), some of these frameworks are model-specific and are implemented on specific models such as decisiont trees~\cite{izza2020explaining}, tree ensembles~\cite{ignatiev2022using} or neural networks~\cite{wu2024verix,bassan2023towards,la2021guaranteed}.

Despite the notable insights that post-hoc approaches provide, they exhibit different problems, such as lack of faithfulness~\cite{rudin2019stop,slack2020fooling,camburu2019can}, scalability issues due to high computational demands~\cite{barcelo2020model,bassan2024local}, and sensitivity to sampling \acrshort{ood} assignments~\cite{hase2021out}. 
To tackle these issues a new line of research has suggested \emph{self explaining neural networks} (SENNs)~\cite{alvarez2018towards} as a general framework under which one can train a model that inherently provides explanations as part of its input, and thus mitigating some of these prior problems. Self-explaining models inherently provide \emph{additive feature attributions}, assigning importance weights to individual or high-level features. 
For instance, Chen et al.~\cite{chen2019looks} and Wang et al.~\cite{wang2021self} describe model outputs by comparing them to relevant “prototypes,” while Alvarez et al.~\cite{alvarez2018towards} derive concept coefficients through feature transformations. 
Other methods, such as those proposed by Agarwal et al.~\cite{agarwal2021neural} and Jain et al.~\cite{jain2020learning}, focus on feature-specific neural networks or use classifiers applied to text snippets for NLP explanations. 
Additionally, Koh et al.~\cite{koh2020concept} predict outcomes based on high-level concepts. 
A recent work by Bassan et al.~\cite{bassan2025iclr} proposes a self-explaining architecture that inherently generates sufficient explanations for its predictions.


%This is particularly important in safety critical tasks, such as in 
%It serves multiple purposes~\cite{meske2022explainable,adadi2018peeking}, one of which is increasing trust and accountability in \acrshort{ai} (and thus in \acrshort{ml}) -based systems. 


%\acrshort{xai} can take on many forms, as evident in the useful taxonomy proposed by Arya et al.~\cite{arya2019one}.
%In recent years, much effort has been put into local self-explaining \acrshort{xai} approaches.
%Such approaches include incorporating pre-existing human-generated explanations into the training~\cite{hind2019ted}, feature-attribution using attention mechanisms~\cite{wickramanayake2022building}, 
%and a feature-attribution method that favors attribution of foreground pixels over background pixels~\cite{chefer2022optimizing}, to name a few.
%However, much of these works, as is the work on \acrshort{xai} in general, are not supported by formal guarantees of rigor. 
%Marques-Silva used the term \textit{non-formal \acrshort{xai}} and critically assessed it~\cite{marques2023disproving}.


%Conversely, \textit{formal \acrshort{xai}} builds on formally defined notions of explainability, such as sufficient reasons.
% One example is incorporating pre-existing human-generated explanations into the training, as done in~\cite{hind2019ted}.
% While this approach focuses on human-understandable explanations, very seldom would one have access to data with both labels and explanations.
% Another example is feature-attribution using attention mechanisms, as presented in~\cite{wickramanayake2022building}.
% This approach provides insight into the inner workings of the model, but it does not leverages any form of exaplainability in the model's training.
% That is, it adds built-in explanations to the model, but the model is trained to optimize performance.
% In ~\cite{chefer2022optimizing} Chefer et al. presented a method that favors attribution of foreground pixels over background pixels.
% While this approach trains the model on an explanation-related objective in addition to performance, it is specific to vision and cannot be applied to other domains, such as \acrshort{bpm}.
%Sufficient reasons are subsets of the input features that suffice to get the same prediction as the original input by the explained \acrshort{ml} model. 
%That is, fixing the values of these features and changing the rest of the features - within reason - will result in the same prediction by the model.
%Assuming a deterministic \acrshort{ml} model, the complete set of the input features would constitute a sufficient reason.
%However, such explanation would not be very informative and, therefore, usually, a desideratum of minimality is added, as a minimal explanation is typically assumed to provide a better interpretation~\cite{barcelo2020model,ribeiro2018anchors,ignatiev2019abduction,ribeiro2016should,waldchen2021computational}.
%Anchors~\cite{ribeiro2018anchors} and SIS~\cite{carter2019made} are a couple of examples for post-hoc techniques that seek the smallest possible sufficient reason.

% \acrshort{xai} methods can be used to make non-interpretable models explainable. 
% Explainable \acrshort{ml} models are models whose inner workings are not human-understandable, but can be explained using proxies (e.g., feature importance of surrogate interpretable models [34, 26]).
% Generally speaking, \acrshort{xai} methods for \acrshort{ml} models can be categorized into local, global, and hybrid methods. 
% Local explanation methods, such as \acrfull{lime} [34] or \acrfull{shap} [26], provide an explanation for a specific model prediction. 
% These methods usually provide an explanation in the form of a list. This list can indicate, for example, the respective contribution of each of the features to the particular prediction or alternative values that would result in a different prediction (i.e., counterfactual explanation). 
% In contrast, global \acrshort{xai} methods explain a \acrshort{ml} model over the entire input space, as captured by the training data. 
% Hybrid methods explain a \acrshort{ml} model over sub-samples of the input space. 
% In this paper we focus on adjusting the global explanation provided by XRF models to accommodate the user’s FP.

% \subsection{Sufficient Reasons}

\subsection{Predictive Business Process Monitoring}
%
% NAP before DL
\acrshort{pbpm} tasks, including \acrshort{nap}, have been studied for several decades. 
Initially, classical \acrshort{ml} methods were applied to these tasks; \cite{marquez2017survey} surveyed these techniques. 
Typically, \acrshort{ml} methods, including \acrlongpl{svm}, Decision Trees, Random Forests, and others, perform well with numeric and categorical attributes but struggle to incorporate sequential data seamlessly.  

% DL and LSTM
With the advent of \acrshort{dl}, \acrshort{lstm} emerged as the predominant approach to \acrshort{pbpm} for several years. 
One of the earliest applications of \acrshort{lstm} to \acrshort{nap} was presented in \cite{evermann2017DL}. 
Using the work of ~\cite{evermann2017DL} as a baseline, ~\cite{tax2017lstm} suggested an alternative \acrshort{lstm} architecture and achieved superior results on  benchmark datasets. 
In our work, we utilize the algorithm and implementation from \cite{tax2017lstm} as a starting point.  
For additional details, there are comprehensive reviews of \acrshort{dl} applications to \acrshort{pbpm} ~\cite{neu2021prediction,ramamaneiro2023benchmark,ramamaneiro2024graph}. 
% A comprehensive review of \acrshort{dl} applications to \acrshort{pbpm}, along with discussions on various aspects of the prediction pipeline such as feature engineering and encoding, can be found in \cite{neu2021prediction}. 
% In addition to another related art survey, \cite{ramamaneiro2023benchmark} includes a benchmark study wherein several algorithms with available code in the open domain are executed and compared across multiple benchmark datasets. 
% Further enhancing the benchmark study in \cite{ramamaneiro2023benchmark}, \cite{ramamaneiro2024graph} introduces a novel prediction algorithm that employs graph convolutional networks embedded in a \acrfull{rnn}.

% Transformer-based research
% Recently, transformer-based architectures \cite{vaswani2017attention} have become a popular approach to \acrshort{pbpm} and \acrshort{nap}~\cite{philipp2020attention,chen2022multi,ni2023transformer}. 
% These methods, trained on large-scale corpora of text data, have led to the development of language \acrshortpl{fm}~\cite{oved2024snap}. 

% For example, one prediction approach uses \acrshortpl{fm} to allow for the integration of textual features and semantic context found in business process logs~\cite{oved2024snap}. 
% It transforms historical data into textual semantic stories, replacing a classical approach of numerical feature matrices.

The recent emphasis on trustworthiness in \acrshort{ai} systems has spurred research into explainability within the \acrshort{pbpm} domain. 
For example, SHAP~\cite{lundberg2017unified} can be leveraged to obtain explanations for \acrlong{kpi} predictions, such as remaining time and activity execution~\cite{galanti2020explainable}.
In another example, feature attribution explainability was incorporated into the prediction algorithm~\cite{wickramanayake2022building}. To the best of our knowledge, this is the first work to propose a self-explaining architecture in the PBPM domain.

% The recent emphasis on trustworthiness in \acrshort{ai} systems has spurred research into explainability and causality within the \acrshort{pbpm} domain. 
% For example, Shapley values can be leveraged to obtain explanations for \acrlong{kpi} predictions, such as remaining time and activity execution~\cite{galanti2020explainable}, and causal \acrshort{ml} techniques can be used to explore which actions yield the highest causal effect on business process outcomes~\cite{bozorgi2020causal}. 
% While the examples above utilize post-hoc explanations, \cite{wickramanayake2022building} incorporated feature attribution explainability into the prediction algorithm. 
% In the current work we propose a minimal sufficient explanation approach which identifies a feature set that determines the prediction, rather than the individual contribution of features to a prediction. 

% Galanti et al.  \cite{galanti2020explainable} demonstrated how explanations can be provided in the  \acrshort{pbpm} field by leveraging Shapley values to obtain explanations for \acrlong{kpi} predictions, such as remaining time and activity execution. 
% Bozorgi et al. \cite{bozorgi2020causal} applied causal \acrshort{ml} techniques to the \acrshort{bpm} domain, exploring which actions yield the highest causal effect on business process outcomes. 
% However, the research above is focused on post-hoc explanations. 
% In contrast, the prediction approach in \cite{wickramanayake2022building} incorporates explainability into the prediction algorithm. 
% However, the feature attribution method presented therein differs from our research. 
% While the feature attribution method of \cite{wickramanayake2022building} identifies which features influenced predictions more than others, our minimal sufficient explanation approach identifies a feature set that determines the prediction and cannot be reduced further.  

